Scheduling Resource-Bounded Monitoring Devices for Event Detection and Isolation in Networks

In networked systems, monitoring devices such as sensors are typically deployed to monitor various target locations. Targets are the points in the physical space at which events of some interest, such as random faults or attacks, can occur. Most often, these devices have limited energy supplies, and they can operate for a limited duration. As a result, energy-efficient monitoring of various target locations through a set of monitoring devices with limited energy supplies is a crucial problem in networked systems. In this paper, we study optimal scheduling of monitoring devices to maximize network coverage for detecting and isolating events on targets for a given network lifetime. The monitoring devices considered could remain active only for a fraction of the overall network lifetime. We formulate the problem of scheduling of monitoring devices as a graph labeling problem, which unlike other existing solutions, allows us to directly utilize the underlying network structure to explore the trade-off between coverage and network lifetime. In this direction, first we propose a greedy heuristic to solve the graph labeling problem, and then provide a game-theoretic solution to achieve near optimal graph labeling. Moreover, the proposed setup can be used to simultaneously solve the scheduling and placement of monitoring devices, which yields improved performance as compared to separately solving the placement and scheduling problems. Finally, we illustrate our results on various networks, including real-world water distribution networks.

==> Introduction.tex <==
Detection and identification of faults in physical systems and processes is fundamental in a variety of practical applications.
For example, leakage detection in water-distribution networks can reduce physical damage as well as financial losses. \todo{Add numbers on losses and references!}
%Monitoring physical systems and processes is of critical importance in a variety of practical applications.
%Reliable control of non-deterministic processes hinges on our ability to measure the processes.
However, in spatially-distributed, networked cyber-physical systems (CPSs), monitoring can prove to be a challenging task.

Systems distributed over large areas may often be monitored only by battery-powered devices, as wired deployment can be prohibitively expensive or simply impossible.
If the power supply provided by batteries is insufficient for continuous monitoring during the intended lifetime of a system, which can be years or even decades for some CPS, batteries must be replaced regularly.
Since the cost of battery replacement for a large number of devices can be very expensive, one of the primary design concerns for such systems is increasing lifetime, that is, increasing the time until the batteries of the sensors are depleted.

One of the primary approaches for conserving battery power is ``sleep scheduling.''
The idea behind this approach is to have only a subset of the sensors activated at any given time, and to turn off (i.e., ``sleep'') the remaining ones, thereby conserving power.
By activating different sets of devices one after another, the lifetime of a system can be substantially increased.
Previous work has focused on finding schedules that ensure complete coverage, that is, guaranteeing that every target is monitored by some device at any given moment in time. \todo{Add some citations to previous work on complete coverage!}
However, complete coverage is a very strict requirement, which severely limits the sets of devices that may be asleep at the same time.
In fact, coverage (i.e., ratio of monitored targets) is a submodular function of the set of active devices in most models, which that attaining completely coverage is disproportionally expensive compared reasonably good coverage. \todo{Do we want to make this argument?}

In this paper, we relax this requirement and consider schedules that attain good coverage, while further increasing lifetime.
Our approach is most closely related to the work of Wang et al.~\cite{wang2009optimization}.
However, we ... \todo{What is the main difference?}

Our main contributions are the following:
\begin{itemize}
\item TODO
\end{itemize} 
Furthermore, the graph-labeling results presented in this paper could have many more applications.

The remainder of this paper is organized as follows.
In Section~\ref{sec:model}, we ...


==> Simultaneous_Selection.tex <==
\section{Simultaneous Placement and Scheduling of Monitoring Devices}
\label{sec:simultaneous}
%\todo{I think a relatively simple solution would be extending the action space with an empty set of labels, and defining the utilities to be zero when the number of players with a non-empty label set is above a constant.}



\subsection{Examples}

